Disparate Impact of Artificial Intelligence Bias in Ridehailing Economy's Price Discrimination Algorithms

Ridehailing applications that collect mobility data from individuals to inform smart city planning predict each trip's fare pricing with automated algorithms that rely on artificial intelligence (AI). This type of AI algorithm, namely a price discrimination algorithm, is widely used in the industry's black box systems for dynamic individualized pricing. Lacking transparency, studying such AI systems for fairness and disparate impact has not been possible without access to data used in generating the outcomes of price discrimination algorithms. Recently, in an effort to enhance transparency in city planning, the city of Chicago regulation mandated that transportation providers publish anonymized data on ridehailing. As a result, we present the first large-scale measurement of the disparate impact of price discrimination algorithms used by ridehailing applications. The application of random effects models from the meta-analysis literature combines the city-level effects of AI bias on fare pricing from census tract attributes, aggregated from the American Community Survey. An analysis of 100 million ridehailing samples from the city of Chicago indicates a significant disparate impact in fare pricing of neighborhoods due to AI bias learned from ridehailing utilization patterns associated with demographic attributes. Neighborhoods with larger non-white populations, higher poverty levels, younger residents, and high education levels are significantly associated with higher fare prices, with combined effect sizes, measured in Cohen's d, of -0.32, -0.28, 0.69, and 0.24 for each demographic, respectively. Further, our methods hold promise for identifying and addressing the sources of disparate impact in AI algorithms learning from datasets that contain U.S. geolocations.

==> figs/nw_significance.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.25\textwidth]{figs/nw_significance2.png}
    \caption{
    The following heatmap displays the change in combined effect size when each neighborhood is omitted, with darker colors signifying a larger difference in combined effect size, and lighter colors signifying a smaller difference in combined effect size.
    % Many of the most significant\textcolor{red}{revise } neighborhoods lie to the West and Northwest of downtown Chicago, areas where there are relatively fewer dropoffs.
    This tells us how much of a single neighborhood changes the mean fare pricing across the city. 
    Figure~\ref{fig:nw_significance} shows that the disparity in fare pricing between largely white and non-white neighborhoods in Chicago could be due to rides to and from largely white neighborhoods that have relatively low pickup or dropoff frequencies.
    }
    \label{fig:nw_significance}
\end{figure} 
